Bivariate exponential integrals and edge-bicolored graphs

We show that specific exponential bivariate integrals serve as generating functions of labeled edge-bicolored graphs. Based on this, we prove an asymptotic formula for the number of regular edge-bicolored graphs with arbitrary weights assigned to different vertex structures. The asymptotic behavior is governed by the critical points of a polynomial. As an application, we discuss the Ising model on a random 4-regular graph and show how its phase transitions arise from our formula.

==> FigColored/tadpole2_rr.tex <==
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-1.5ex]current bounding box.center)}]
    \coordinate (v);

    \coordinate [above=4 of v] (vm1);
    \coordinate [left=3 of vm1] (v01);
    \coordinate [right=3 of vm1] (v11);
    \draw[cb-red, line width = 3.5] (v01) circle(3);
    \draw[cb-red, line width = 3.5] (v11) circle(3);
    \filldraw (vm1) circle (3pt);
\end{tikzpicture}%

==> FigColored/tadpole2_ry.tex <==
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-1.5ex]current bounding box.center)}]
    \coordinate (v);

    \coordinate [above=4 of v] (vm1);
    \coordinate [left=3 of vm1] (v01);
    \coordinate [right=3 of vm1] (v11);
    \draw[cb-red, line width = 3.5] (v01) circle(3);
    \draw[cb-yellow, line width = 3.5] (v11) circle(3);
    \filldraw (vm1) circle (3pt);
\end{tikzpicture}%

==> FigColored/tadpole2_yy.tex <==
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-1.5ex]current bounding box.center)}]
    \coordinate (v);

    \coordinate [above=4 of v] (vm1);
    \coordinate [left=3 of vm1] (v01);
    \coordinate [right=3 of vm1] (v11);
    \draw[cb-yellow, line width = 3.5] (v01) circle(3);
    \draw[cb-yellow, line width = 3.5] (v11) circle(3);
    \filldraw (vm1) circle (3pt);
\end{tikzpicture}%

==> figs/banana3.tex <==
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-.5ex]current bounding box.center)}]
    \coordinate (vm);
    \coordinate [left=1 of vm] (v0);
    \coordinate [right=1 of vm] (v1);
    \draw (v0) -- (v1);
    \draw (vm) circle(1);
    \filldraw (v0) circle (1pt);
    \filldraw (v1) circle (1pt);
\end{tikzpicture}%


==> figs/banana3_1forest.tex <==
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-.5ex]current bounding box.center)}]
    \coordinate (vm);
    \coordinate [left=1 of vm] (v0);
    \coordinate [right=1 of vm] (v1);
    \draw[col1,thick] (v0) -- (v1);
    \draw (vm) circle(1);
    \filldraw (v0) circle (1pt);
    \filldraw (v1) circle (1pt);
\end{tikzpicture}%


==> figs/banana3withbubble.tex <==
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-.5ex]current bounding box.center)}]
    \coordinate (vm);
    \coordinate [left=1 of vm] (v0);
    \coordinate [right=1 of vm] (v1);
    \coordinate [right=.7 of v1] (o);
    \draw (v0) -- (v1);
    \draw (vm) circle(1);
    \draw (o) circle(.7);
    \filldraw (v0) circle (1pt);
    \filldraw (v1) circle (1pt);
\end{tikzpicture}%


==> figs/handle.tex <==
\begin{tikzpicture}[x=1ex,y=1ex,baseline={([yshift=-.5ex]current bounding box.center)}]
    \coordinate (v0);
    \coordinate [right=1.5 of v0] (v1);
    \coordinate [left=.7 of v0] (i0); 
    \coordinate [right=.7 of v1] (o0); 
    \draw (v0) -- (v1);
    \filldraw (v0) circle (1pt);
    \filldraw (v1) circle (1pt);
    \draw (i0) circle(.7);
    \draw (o0) circle(.7);
\end{tikzpicture}%

